Peeking Behind the Curtains of Residual Learning

The utilization of residual learning has become widespread in deep and scalable neural nets. However, the fundamental principles that contribute to the success of residual learning remain elusive, thus hindering effective training of plain nets with depth scalability. In this paper, we peek behind the curtains of residual learning by uncovering the "dissipating inputs" phenomenon that leads to convergence failure in plain neural nets: the input is gradually compromised through plain layers due to non-linearities, resulting in challenges of learning feature representations. We theoretically demonstrate how plain neural nets degenerate the input to random noise and emphasize the significance of a residual connection that maintains a better lower bound of surviving neurons as a solution. With our theoretical discoveries, we propose "The Plain Neural Net Hypothesis" (PNNH) that identifies the internal path across non-linear layers as the most critical part in residual learning, and establishes a paradigm to support the training of deep plain neural nets devoid of residual connections. We thoroughly evaluate PNNH-enabled CNN architectures and Transformers on popular vision benchmarks, showing on-par accuracy, up to 0.3% higher training throughput, and 2x better parameter efficiency compared to ResNets and vision Transformers.

==> _txt/6_Discussion.tex <==
\section{Visualization Coder Kernels}
\thc{Put this to Appendix.}
% Chances for Pruning

In this section, we visualize the coder weights to provide more insight into plain CNNs.
We analyze the weights of a coder utilized to maintain inputs for 512$\times$512 ConvNet blocks.
To better study the learned structure-preserving representations in auto-encoder, we define a filter norm: $||W||_{\dot, F}^{i, j}=||W^{i, j, :, :}||_{1}=\sum_{x, y}|W^{i, j, x, y}|$ that computes the L-1 norm of each filter in $W$. We apply the channel norm to the encoder weights $W_{enc}$ and decoder weights $W_{dec}$.

Following Young's inequality~\cite{brascamp1976best}, the operator norm of a convolution filter is upper-bounded by its L-1 norm.
Thus, the filter norm matrix can accurately bound the magnitude that one input channel contributes towards another.
In residual connection, the output channel only relates to a single input channel with unit magnitude.
Although this single pattern achieves competitive performance, the learned kernel, in contrast, develops a mixed pattern in Figure \ref{fig:vis_kernels} that provides the following insights.

\begin{figure}[t]
\begin{center}
    \vspace{-0.5em}
    \includegraphics[width=1.0\linewidth]{_figs/VisKernel.pdf}
    \vspace{-2em}
    \caption{\textbf{(Top)} Filter norm matrix on learned coder. 
    \textbf{(Bottom)}
    Filter norm matrix on identity mapping.
    Here, we visualize the coder dedicated for $C_{in}=512$ ConvCoder blocks.}
    \vspace{-2em}
\label{fig:vis_kernels}
\end{center}
\end{figure}
\noindent $\bullet$ \textbf{Input Importance Varies.} In the learned coder, the row filter norm of encoder weight $W_{enc}$ demonstrates that some input channels might be more relevant to the critical features contained in data.
As a result, these channels adopt a higher filter norm to indicate more influence on outputs.
Contrary to residual connection where each channel is of the same importance, the coder kernel adopts an implicit attention mechanism to accommodate different levels of features and thus, achieves better generalization.

\noindent $\bullet$ \textbf{Coder Promotes Model Compression.} 
In existing model compression literature such as pruning~\cite{luo2020neural}, the residual branch is more difficult to achieve high compression rate.
We observe that a residual connection shows different distribution with convolver weights when represented in coder.
Our hypothesis is that the `uniformly distributed' and non-trainable residual connection in coder may conflict with the Gaussian-distributed convolver, thus results in more difficulty pruning.
With a fully trainable coder which can adapt with the change of convolver weights, we envision that ConvCoder architecture provides a better chance to overcome the limit of model compression. 
